DCID: Deep Canonical Information Decomposition

We consider the problem of identifying the signal shared between two one-dimensional target variables, in the presence of additional multivariate observations. Canonical Correlation Analysis (CCA)-based methods have traditionally been used to identify shared variables, however, they were designed for multivariate targets and only offer trivial solutions for univariate cases. In the context of Multi-Task Learning (MTL), various models were postulated to learn features that are sparse and shared across multiple tasks. However, these methods were typically evaluated by their predictive performance. To the best of our knowledge, no prior studies systematically evaluated models in terms of correctly recovering the shared signal. Here, we formalize the setting of univariate shared information retrieval, and propose ICM, an evaluation metric which can be used in the presence of ground-truth labels, quantifying 3 aspects of the learned shared features. We further propose Deep Canonical Information Decomposition (DCID) - a simple, yet effective approach for learning the shared variables. We benchmark the models on a range of scenarios on synthetic data with known ground-truths and observe DCID outperforming the baselines in a wide range of settings. Finally, we demonstrate a real-life application of DCID on brain Magnetic Resonance Imaging (MRI) data, where we are able to extract more accurate predictors of changes in brain regions and obesity. The code for our experiments as well as the supplementary materials are available at https://github.com/alexrakowski/dcid

==> acros.tex <==
\newacro{r.v.}{random variable}
\newacroplural{r.v.}[r.v.s]{random variables}
\newacro{MSE}{Mean Squared Error}
\newacro{DNN}{Deep Neural Network}
\newacroplural{DNNs}{Deep Neural Networks}
\newacro{CNN}{Convolutional Neural Network}
\newacro{ML}{Machine Learning}
\newacro{ML4H}{Machine Learning for Health}
\newacro{DL}{Deep Learning}
\newacro{AI}{Artificial Intelligence}
\newacro{MRI}{Magnetic Resonance Imaging}
\newacroplural{MRI}[MRIs]{Magnetic Resonance Images}
\newacro{GAN}{Generative Adversarial Network}
\newacroplural{GAN}[GANs]{Generative Adversarial Networks}
\newacro{VAE}{Variational Autoencoder}
\newacroplural{VAE}[VAEs]{Variational Autoencoders}
\newacro{MLE}{Maximum Likelihood Estimation}
\newacro{MI}{Mutual Information}
\newacro{PCA}{Principal Component Analysis}
\newacro{CCA}{Canonical Correlation Analysis}
\newacro{ICA}{Independent Component Analysis}
\newacro{ROI}{Region of Interest}
\newacroplural{ROI}[ROIs]{Regions of Interest}
\newacro{CT}{Computed tomography}
\newacro{DCID}{Deep Canonical Information Decomposition}
\newacro{pCCA}{Probabilistic CCA}
\newacro{MTL}{Multi-Task Learning}
\newacro{Adv. MTL}{Adversarial Multi-Task Learning}
\newacro{MTFL}{Multi-Task Feature Learning}

\newacro{CSF}{cerebrospinal fluid}
\newacro{BFM}{body fat mass}
\newacro{BMI}{body mass index}
\newacro{UKB}{UK Biobank}
\newacro{ADNI}{Alzheimer's Disease Neuroimaging Initiative}
\newacro{AD}{Alzheimer's Disease}

\newacro{CDR}{Clinical Dementia Rating}

\newacro{t.v.}{target variable}
\newacroplural{t.v}[t.v.s]{target variables}

\newacro{g.t.}{ground-truth}
\newacro{SPM}{Statistical Parametric Mapping}
\newacroplural{SPM}[SPMs]{Statistical Parametric Mappings}

\newacro{DAG}{Directed Acyclic Graph}
\newacro{SotA}{state-of-the-art}
\newacro{CMI}{Conditional Mutual Information}
% TODO
\newacro{BRNet}{BRNet}
% TODO
\newacro{CNC}{Correct-N-Contrast}
\newacro{ECE}{Expected Calibration Error}
\newacro{IRM}{Invariant Risk Minimization}
